Extreme Memorization via Scale of Initialization

We construct an experimental setup in which changing the scale of initialization strongly impacts the implicit regularization induced by SGD, interpolating from good generalization performance to completely memorizing the training set while making little progress on the test set. Moreover, we find that the extent and manner in which generalization ability is affected depends on the activation and loss function used, with $\sin$ activation demonstrating extreme memorization. In the case of the homogeneous ReLU activation, we show that this behavior can be attributed to the loss function. Our empirical investigation reveals that increasing the scale of initialization correlates with misalignment of representations and gradients across examples in the same class. This insight allows us to devise an alignment measure over gradients and representations which can capture this phenomenon. We demonstrate that our alignment measure correlates with generalization of deep models trained on image classification tasks.

==> concentration.tex <==

\section{Covariance Bound for Gradient Descent}

In this section we consider the operation of gradient descent on smooth loss functions. We identify the average correlation over all examples of the example gradients with the true mean gradient of the loss as a measure of quality of the gradient descent step: when this quantity is close to the norm of the mean gradient squared, then we can be confident that gradient descent is taking ``safe'' steps in the sense that the test loss will not be increasing.

In order to setup our analysis, we need a few assumptions and definitions. We consider a function $f:\R^d\to \R$ to be $G$-Lipschitz if $\|\nabla f(x)\|\le G$ for all $x$. $f$ is said to be $L$-smooth if $\|\nabla^2f(x)\|_{\text{op}}\le L$ for all $x\in \R^d$. This also implies by Taylor's theorem that for all $x,y$, $f(x) \le f(x) + \nabla f(x)\cdot (x-y) +\frac{L}{2}\|x-y\|^2$. We suppose that there is some (unknown) distribution $D$ over $L$-smooth and $G$-Lipschitz functions, and we have a ``dataset'' of $N$ i.i.d. draws from this distribution $f_1,\dots,f_N$. Our objective is to find a point that minimizes $F(x)=\E_{f\sim D}[f(x)]$. In practice, each $f_i$ represents the loss of the network parameters $x$ on the $i$th example in the training set. We define the training loss as $\hat F(x) = \frac{1}{N}\sum_{i=1}^N f_i(x)$.

Gradient descent starts with an initial iterate $x_0\in \R^d$ and repeatedly generates new iterates via the recursive formula:
\begin{align*}
    x_{t+1} = x_t - \eta \nabla F(x_t)
\end{align*}
for some parameter $\eta\in \R$.

We can prove the following statement about one step of gradient descent:
\begin{Theorem}\label{thm:onestepgd}
Given an iterate $x_t$, Let $\Sigma$ be the covariance matrix of $\nabla f(x_t)$: $\Sigma = \E[\nabla f(x_t)\nabla f(x_t)^\top] - \nabla F(x_t)\nabla F(x_t)^\top$. Then, with probability at least $1-\delta$:
\begin{align*}
    F(x_{t+1}) \le F(x_t) - \eta \|\nabla F(x_t)\|^2 +\eta\frac{4\sqrt{\nabla F(x_t)^\top \Sigma\nabla F(x_t)\log(1/\delta)}}{\sqrt{N}} + \eta\frac{2G\|\nabla F(x_t)\|\log(2/\delta)}{3N} + \frac{L\eta^2G^2}{2}
\end{align*}
\end{Theorem}
\begin{proof}
Define $\epsilon = \nabla\hat F(x_t) - \nabla F(x_t)$.
By smoothness, we have
\begin{align*}
    F(x_{t+1})&\le F(x_t) - \eta \langle \nabla \hat F(x_t),\nabla F(x_t)\rangle +\frac{L\eta^2\|\nabla \hat F(x_t)\|^2}{2}\\
    &\le F(x_t) - \eta \|\nabla F(x_t)\|^2 -\eta \langle \epsilon , \nabla F(x_t)\rangle + \frac{L\eta^2G^2}{2}
\end{align*}
Thus the result requires that we bound $\langle \epsilon,\nabla F(x_t)\rangle$ with high probability. To do this, define $\epsilon_i = \nabla f_i(x_t) - \nabla F(x_t)$. Then we have that $\E[\epsilon_i\epsilon_i^\top] = \Sigma$. 
\begin{align*}
    \langle \epsilon,\nabla F(x_t)\rangle = \frac{1}{N}\sum_{i=1}^N\langle \epsilon_i , \nabla F(x_t)\rangle
\end{align*}
Observe that $\langle \epsilon_i, \nabla F(x_t)\rangle$ is mean-zero random variable satisfying $\langle \epsilon_i, \nabla F(x_t)\rangle\le G\|\nabla F(x_t)\|$, and has variance $\nabla F(x_t)^\top \Sigma \nabla F(x_t)$. Therefore, by Bernstein's inequality:
\begin{align*}
    \text{Prob}\left[-\sum_{i=1}^N\langle \epsilon_i , \nabla F(x_t)\rangle\ge z\right]\le \exp\left(-\frac{z^2}{2N\nabla F(x_t)^\top \Sigma \nabla F(x_t) + 2G\|\nabla F(x_t)\|z/3}\right)
\end{align*}
So that we have with probability at least $1-\delta$:
\begin{align*}
    -\sum_{i=1}^N\langle \epsilon_i , \nabla F(x_t)\rangle \le 4\sqrt{N\nabla F(x_t)^\top \Sigma \nabla F(x_t)\log(1/\delta)} + \frac{2G\|\nabla F(x_t)\|\log(1/\delta)}{3}
\end{align*}
and dividing by $N$ yields the Theorem.
\end{proof}

In order to analyze the performance of gradient descent , we will make use of the following complexity definitions:
\begin{Definition}\label{dfn:covariance}
The \emph{covariance complexity} of a set $X\subset \R^d$ with respect to the distribution $D$ is:
\begin{align*}
    C(X,D, N)=\E_{f_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N \left\langle \nabla f_i(x)-\nabla F(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]
\end{align*}
where  the expectation is over the sample $f_i$.

\end{Definition}

\begin{Definition}\label{dfn:empcovariance}
The \emph{normalized empirical covariance complexity} at a point $x$ is:
\begin{align*}
    NEC(x)=\frac{\frac{1}{N}\sum_{i=1}^N \left\langle \nabla f_i(x)-\nabla \hat F(x), \frac{\nabla \hat F(x)}{\|\nabla \hat F(x)\|}\right\rangle}{\|\nabla \hat F(x)\|}
\end{align*}
where recall we define:
\begin{align*}
    \hat \nabla F(x) = \frac{1}{N}\sum_{i=1}^N \nabla f_i(x)
\end{align*}
\end{Definition}


\begin{Definition}\label{dfn:rademacher}
The \emph{rademacher covariance complexity} of a set $X\subset \R^d$ with respect to the distribution $D$ is:
\begin{align*}
    R(X,D, N)=\E_{f_i,\sigma_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N \left\langle \sigma_i \nabla f_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]
\end{align*}
where $\sigma_1,\dots,\sigma_N$ are i.i.d. Rademacher signs, and the expectation is over both the $\sigma_i$ and the $f_i$.
\end{Definition}

\begin{Definition}\label{dfn:rademacher}
The \emph{empirical rademacher covariance complexity} of a set $X\subset \R^d$ at a point $x$ is
\begin{align*}
    ER(x)=\frac{\frac{1}{\sqrt{N}}\sum_{i=1}^N \left\langle \sigma_i \nabla f_i(x), \frac{\nabla \hat F(x)}{\|\nabla \hat F(x)\|}\right\rangle}{\|\nabla \hat F(x)\|}
\end{align*}
where $\sigma_1,\dots,\sigma_N$ are i.i.d. Rademacher signs.
\end{Definition}

With this in hand, we can generalize Theorem \ref{thm:onestepgd} to many steps of gradient descent through a symmetrization argument:
\begin{Theorem}\label{thm:rademachergd}
Suppose that the iterates $x_t$ lie in some region $X$ with probability 1 (e.g. $X$ is certainly contained in the ball of radius $T\eta G$ centered at $x_0$). Then we have:
\begin{align*}
    \E[F(x_{T+1}])\le F(x_0)-\frac{\eta}{2} \sum_{t=1}^T \E[\|\nabla F(x_t)\|^2] + \frac{\eta T C(X,D,N)}{2N^2}+\frac{\eta^2 T LG^2}{2} 
\end{align*}
Further, we have
\begin{align*}
    C(X,D,N)\le 4 R(X,D,N)
\end{align*}
\end{Theorem}
\begin{proof}
Define $\epsilon_i(x) = \nabla f_i(x) - \nabla F(x)$ and $\epsilon(x) = \frac{1}{N}\sum_{i=1}^N \epsilon_i(x)$. Then by smoothness, we have:
\begin{align*}
    \E[F(x_{t+1})] &= \E[F(x_t)] - \eta \E[\|\nabla F(x_t)\|^2] - \eta \E[\|\nabla F(x_t)\|\langle \epsilon(x_t), \frac{\nabla F(x_t)}{\|\nabla F(x_t)\|}\rangle] + \frac{\eta^2 LG^2}{2}\\
    &\le \E[F(x_t)] - \frac{\eta}{2} \E[\|\nabla F(x_t)\|^2] - \frac{\eta}{2} \E[\langle \epsilon(x_t), \frac{\nabla F(x_t)}{\|\nabla F(x_t)\|}\rangle^2] + \frac{\eta^2 LG^2}{2}\\
    \E[F(x_{T+1})]&\le F(x_0) - \frac{\eta}{2} \sum_{t=1}^T \E[\|\nabla F(x_t)\|^2]+\frac{\eta}{2}\E[\sum_{t=1}^T\langle \epsilon(x_t), \frac{\nabla F(x_t)}{\|\nabla F(x_t)\|}\rangle^2] +\frac{\eta^2 T LG^2}{2}\\
    &\le  F(x_0) - \frac{\eta}{2} \sum_{t=1}^T \E[\|\nabla F(x_t)\|^2]+\frac{\eta T}{2}\E[\sup_{x\in X}\langle \epsilon(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\rangle^2] +\frac{\eta^2 T LG^2}{2}
\end{align*}
Now observe that $\E[\sup_{x\in X}\langle \epsilon(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\rangle^2]$ is by definition $\frac{C(X,D,N)}{N^2}$.

Now we prove the relationship between $C(X,D,N)$ and $R(X,D,N)$. To this end, let $f'_1,\dots,f'_N$ be a ghost dataset drawn from the same distribution $D$. Also let $\sigma_1,\dots,\sigma_N$ be independent Rademacher random variables.
\begin{align*}
    C(X,D<N)&=\E_{f_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla F(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
    &=\E_{f_i}\left[\sup_{x\in X}\left(\E_{f'_i}\left[\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right]\right)^2\right]\\
    &=\E_{f_i,\sigma_i}\left[\sup_{x\in X}\left(\E_{f'_i}\left[\sum_{i=1}^N\left\langle \sigma_i(\nabla f_i(x) - \nabla f'_i(x)), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right]\right)^2\right]\\
    &=\E_{f_i,f'_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
    &=\E_{f_i,f'_i,\sigma_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \sigma_i (\nabla f_i(x)-\nabla f'_i(x)), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
    &\le \E_{f_i,f'_i,\sigma_i}\left[\sup_{x\in X}2\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right.\\
    &\quad\quad\quad\quad\quad\quad\quad\quad+\left. 2\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
    &=4 \E_{f_i, \sigma_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
    &=4 R(X,D,N)
\end{align*}


Let us unpack the statement of Theorem \ref{thm:rademachergd}. First, consider the case that the training set perfectly captures the true distribution, so that training error equals testing error. In this case, we have $C(X,D,N)=0$ and so the result decays to
\begin{align*}
    F(x_{T+1}\le F(x_0)-\frac{\eta}{2} \sum_{t=1}^T \|\nabla F(x_t)\|^2 +\frac{\eta^2 T LG^2}{2} 
\end{align*}
which is a standard convergence guarantee for gradient descent. Next, notice that by a simple covering argument, we have that $C(X,D,N)=\tilde O($
% alternate try:

% \begin{align*}
%     \E_{f_i}\left[\sup_{x\in X}\left\langle \epsilon(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle^2\right]&=\E_{f_i}\left[\sup_{x\in X}\left(\frac{1}{N}\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla F(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
%     &=\frac{1}{N^2}\E_{f_i}\left[\sup_{x\in X}\left(\E_{f'_i}\left[\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right]\right)^2\right]\\
%     &=\frac{1}{N^2}\E_{f_i,\sigma_i}\left[\sup_{x\in X}\left(\E_{f'_i}\left[\sum_{i=1}^N\left\langle \sigma_i(\nabla f_i(x) - \nabla f'_i(x)), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right]\right)^2\right]\\
%     &=\frac{1}{N^2}\E_{f_i,\sigma_i}\left[\sup_{x\in X}\E_{f'_i}\left(\left[\sum_{i=1}^N\left\langle \sigma_i(\nabla f_i(x) - \nabla f'_i(x)), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right]\right)^2-\mathop{\text{Var}}_{f'_i}\left(\sum_{i=1}^N \left\langle \sigma_i f'_i,\frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)\right]\\
%     &=\frac{1}{N^2}\E_{f_i,f'_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2-\mathop{\text{Var}}_{f_i}\left(\sum_{i=1}^N \left\langle \sigma_i f_i,\frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)\right]\\
%     &=\frac{1}{N^2}\E_{f_i,f'_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \nabla f_i(x) - \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
%     &=\frac{1}{N^2}\E_{f_i,f'_i,\sigma_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \sigma_i (\nabla f_i(x)-\nabla f'_i(x)), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
%     &\le \frac{1}{N^2}\E_{f_i,f'_i,\sigma_i}\left[\sup_{x\in X}2\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right.\\
%     &\quad\quad\quad\quad\quad\quad\quad\quad+\left. 2\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f'_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
%     &=\frac{4}{N^2} \E_{f_i, \sigma_i}\left[\sup_{x\in X}\left(\sum_{i=1}^N\left\langle \sigma_i \nabla f_i(x), \frac{\nabla F(x)}{\|\nabla F(x)\|}\right\rangle\right)^2\right]\\
%     &=\frac{4 R(X,D,N)}{N^2}
% \end{align*}
\end{proof}



 





\ashok{work in progress... technically this is only about *one* gradient step and quickly becomes problematic for multiple steps. This can be naively fixed via covering arguments, but that may incur a large dimension penalty. One could probably also appeal to some kind of vector rademacher complexity (which is presumably tighter than covering numbers), but this just kicks the can down the road since I have no idea what that rademacher complexity would actually be.}


The main result of this section is the following. Roughly speaking, it says that for small enough $\eta$, there are three regimes of SGD: one in which the training gradient is large and we make fast progress on both training and test loss. However, once the training gradient becomes small enough, then whether we make progress on the test loss depends on the quantity $\sqrt{\frac{\nabla F(x)^\top \Sigma \nabla F(x)}{n}}+\frac{\|\nabla F(x)\|}{n}$ where $n$ is the training set size and $\Sigma$ is the covariance matrix of the gradients. \harsh{I'm curious, does this setup assume any network architecture, activation function ?} \ashok{I'm assuming smoothness so you'd technically need a smooth activation function like softplus or something.} If this is smaller than $O(\|\nabla F(x)\|^2)$, then we make progress. If it is on the same order, then we stop making progress on the test loss. If it is bigger, we might overfit. Regardless, we continue to make progress on the train loss. So in the same order regime, we have a ``memorization'' period.


As a simple example, consider the linear loss $f_i(x) = \ell(\langle x, z_i\rangle)$ where $z_i\in \R^d$ indicates some random feature vector and $\ell$ is a fixed smooth and Lipschitz loss (like softmax loss). Suppose the distribution over $z_i$ is simply a uniform distribution over an orthonormal basis of $\R^d$. Then in a dataset of size $n$, the variance of gradients can easily be $O(1)$, so that a typical analysis would say that if the gradient is $O(1/\sqrt{n})$ (which is likely  true at initialization), it is not safe to take a gradient step without risking overfitting. This is too conservative: on this distribution, any gradient step may memorize the training set, but will never damage performance on the test set. The covariance satisfies $\Sigma \preceq \frac{1}{d}I$ (b/c of Lipschitz property), so $\sqrt{\frac{\nabla F(x)^\top \Sigma \nabla F(x)}{n}}+\frac{\|\nabla F(x)\|}{n}\le \frac{\|\nabla F(x)\|}{\sqrt{dn}}+ \frac{\|\nabla F(x)\|}{n}$. Thus, we can continue to safely take a gradient step unless the gradient is $O(1/\sqrt{dn}+1/n)$, which is significantly better.


\ashok{TODO: come up with example that actually has three regimes}


\begin{Theorem}\label{thm:gradprogress}
Suppose $f_1,\dots,f_n$ are i.i.d. random function from $\R^d\to \R$ with mean $F$.Define $\hat F = \frac{1}{n}\sum_{i=1}^n f_i$ and suppose $F$ and $\hat F$ are $L$-smooth with probability 1 and let $x\in \R^d$. Let $g_i = \nabla f_i(x)$ and let $\eta\in \R$, $\eta\le \frac{1}{L}$. Define $\hat G = \frac{1}{n}\sum_{i=1}^n g_i$ and $G = \nabla F(x)$. Let $\delta>0$. Define $\Sigma = \E[(g_i- G)(g_i- G)^\top]$ and let $\sigma^2_1$ be the largest eigenvalue of $\Sigma$ and let $V$ be the trace of $\Sigma$ (the variance of $g$). Let $\delta>0$. Then with probability at least least $1-\delta$, we have the following:

\begin{align*}
    F(x-\eta\hat G)-F(x)\le O\left(-\eta \|G\|^2 + \eta^2L\frac{V^2\log(d/\delta)}{n}+\eta^2\frac{\log^2(d/\delta)}{n^2}+ \eta \sqrt{\frac{G^\top  \Sigma  G\log(1/\delta)}{n}}+\eta\frac{\|G\|\log(1/\delta)}{n}\right)
\end{align*}
\end{Theorem}

This theorem is a nearly immediate consequence of the following few facts:
\begin{Proposition}\label{thm:gradstep}
For any $L$-smooth function $F:\R^d\to \R$ and $x,\hat G\in \R^d$ and $\eta\in [0,1/2L]$,
\begin{align*}
    F(x- \eta G) - F(x) &\le -\eta \langle \hat G, \nabla F(x)\rangle + \eta^2\frac{L}{2}\|\hat G\|^2\\
    &\le -\eta \langle \hat G, \nabla F(x)\rangle + \frac{\eta}{2}\|\nabla F(x)\|^2 + \eta^2L\|\hat G-\nabla F(x)\|^2
\end{align*}
\end{Proposition}


\begin{Proposition}\label{thm:directionhoeffding}
Let $G$, $\hat G$ and $\Sigma$ be as in Theorem \ref{thm:gradprogress}. Then with probability at least $1-\delta$,
\begin{align*}
    -\langle \hat G, G\rangle +\|G\|^2&\le \sqrt{\frac{2G^\top \Sigma G\log(1/\delta)}{n}} + \frac{\|G\|\log(1/\delta)}{3n}
\end{align*}
\end{Proposition}
\begin{proof}
Let $z_i = \langle -g_i +G,G/\|G\|\rangle$. Notice that $z_i$ is mean-zero and has variance $\frac{1}{\|G\|^2}G^\top \Sigma G$. Further, $\frac{\|G\|}{n}\sum_{i=1}^n z_i =- \langle \hat G, G\rangle +\|G\|^2$. The conclusion then follows from Bennet's inequality, which states that if $\sigma^2$ is the variance of $z_i$, then with probability at least $1-\delta$,
\begin{align*}
    \frac{1}{n}\sum_{i=1}^n z_i - \E[z_i]&\le \sqrt{\frac{2\sigma^2 \log(1/\delta)}{n}} + \frac{\log(1/\delta)}{3n}
\end{align*}
\end{proof}

\begin{Proposition}\label{thm:normedhoeffding}
Let $V^2$ be the trace of $\Sigma$. Then with probability at least $1-\delta$,
\begin{align*}
\|\hat G - G\|\le \frac{2\sqrt{V^2 \log((d+1)/\delta)}}{\sqrt{n}} + \frac{4\log((d+1)/\delta)}{3n}
\end{align*}
\end{Proposition}
\begin{proof}
By the rectangular Matrix Bernstein bound \cite{tropp2012user}, we have that 
\begin{align*}
   \text{Prob}\left[ \|n\hat G - n G\|>t\right]&\le (d+1)\exp\left(-\frac{t^2/2}{nV^2+t/3}\right)\\
   &\le (d+1)\max\left[\exp(-t^2/4nV^2), \exp(-3t/4)\right]
\end{align*}
Setting the RHS less than $\delta$, and solving for $t$, we have
\begin{align*}
    t\le 2\sqrt{nV^2 \log((d+1)/\delta)} + \frac{4}{3}\log((d+1)/\delta)
\end{align*}
from which the result follows
\end{proof}

\subsection{Empirical Version... not clear how valuable this is}

This next theorem provides an ``empirical'' version of the previous theorem: now basically all the ``error'' quantities involved are actually measurable with the training data. 
\begin{Theorem}\label{thm:empiricalgradprogress}
Suppose $f_1,\dots,f_n$ are i.i.d. random functions from $\R^d\to \R$ with mean $F$. Define $\hat F = \frac{1}{n}\sum_{i=1}^n f_i$ Suppose $f_i$ is $L$-smooth with probability 1, and let $x\in \R^d$. Let $g_i = \nabla f_i(x)$ and let $\eta\in \R$, $\eta\le \frac{1}{L}$. Define $\hat G = \frac{1}{n}\sum_{i=1}^n g_i$ and $G = \nabla F(x)$. Let $\delta>0$. Define $V = \frac{1}{n-1}\sum_{i=1}^n \|g_i-\hat G\|^2$ and $\hat \Sigma = \frac{1}{n-1}\sum_{i=1}^n(g_i-\hat G)(g_i-\hat G)^\top$. Let $\sigma^2_1$ be the largest eigenvalue of $\hat \Sigma$.

There exists a quantity $z$ with 
\begin{align*}
    z = O\left(\sqrt{\frac{V\log(n/\delta)}{n}} + \frac{\log(n/\delta)}{n}\right)
\end{align*}
such that with probability at least $1-\delta$, we have the following:

\begin{itemize}
    \item if $\|\hat G\|\ge 3z$, then
    \begin{align*}
        F(x-\eta\hat G)-F(x)&\le O(-\eta \|G\|^2)
    \end{align*}
    \item Otherwise, 
    \begin{align*}
      &F(x-\eta\hat G)-F(x)\le O\left(-\eta \|G\|^2 + \eta^2L\frac{V\log(n/\delta)}{n} + \eta^2L\frac{\log^2(n/\delta)}{n^2} + \eta \sqrt{\frac{\hat G^\top \hat \Sigma \hat G\log(1/\delta)}{n}}+\eta \frac{\|G\|\log(1/\delta)}{n} \right.\\
        &\quad \quad\left.+\eta\frac{\sqrt{\|\hat G\|\sigma^2_1\sqrt{V\log(n/\delta)}}}{n^{3/4}}+\eta\frac{\sqrt{\|\hat G\|\sigma^2_1\log(n/\delta)}}{n} +\eta\frac{\sqrt{V\sigma^2_1 \log(n/\delta)}}{n} +\eta \frac{\sqrt{\sigma^2_1} \log(n/\delta)}{n^{3/2}} \right)
    \end{align*}
\end{itemize}
Further, regardless we have
\begin{align*}
    \hat F(x-\eta \hat G) - \hat F(x) \le O(-\eta \|\hat G\|^2)
\end{align*}
\end{Theorem}


A few facts about concentration of empirical gradient estimates to their mean

The following is a corollary of the empirical Bernstein bound \cite{Maurer2009EmpiricalBB}.
\begin{Theorem}\label{thm:covariance}
Suppose $g_1,\dots,g_n$ are i.i.d. samples from a distribution over $d$-dimensional real vectors such that $\|g\|\le 1$ with probability 1. Let $\E[g]=G$, and let $\frac{1}{n}\sum_{i=1}^n g_i = \hat G$. Define the empirical covariance matrix $\hat \Sigma = \frac{1}{n-1}\sum_{i=1}^n (g_i -\hat G)(g_i -\hat G)^\top=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n}(g_i-g_j)(g_i-g_j)^\top$. Let $\sigma^2_1$ be the maximum eigenvalue of $\hat \Sigma$. Then for any $\delta>0$, with probability at least $1-\delta$,
\begin{align*}
    \left|\langle G, \hat G\rangle -\|G\|^2\right|&\le\sqrt{\frac{4G^\top \hat \Sigma G\log(4/\delta)}{n}}+\frac{7\|G\|\log(4/\delta)}{3(n-1)}\\
    &\le \|G\|\sqrt{\frac{4\sigma^2_1\log(4/\delta)}{n}}+\frac{7\|G\|\log(4/\delta)}{3(n-1)}
\end{align*}
\end{Theorem}
\begin{proof}
Define the random variable $x_i = \langle g_i, G/\|G\|\rangle$. Notice that $\langle G, \hat G\rangle = \frac{\|G\|}{n}\sum_{i=1}^n x_i$, and that $\|G\|^2 = \frac{\|G\|}{n}\E[\sum_{i=1}^n x_i]$. Then if we define the sample variance $V=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n}(x_i-x_j)^2$. Then by \cite{Maurer2009EmpiricalBB} Theorem 4 and a union bound, with probability at least $1-\delta$ we have
\begin{align*}
    \left| \frac{1}{n}\sum_{i=1}^n x_i-\|G\|\right|\le \sqrt{\frac{4V\log(4/\delta)}{n}}+\frac{7\log(4/\delta)}{3(n-1)}
\end{align*}
Now, multiply by $\|G\|$ and notice that $\|G\|^2V = G^\top \hat \Sigma G\le \|G\|^2\sigma^2_1$ to complete the proof.
\end{proof}

Another simple corollary (the dimension factor here is annoying...).
\begin{Theorem}\label{thm:dimvariance}
Suppose $g_1,\dots,g_n$ are i.i.d. samples from a distribution over $d$-dimensional real vectors such that $\|g\|\le 1$ with probability 1. Let $\E[g]=G$, and let $\frac{1}{n}\sum_{i=1}^n g_i = \hat G$. Let $V = \frac{1}{n-1}\sum_{i=1}^n \|g_i-\hat G\|^2=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n} \|g_i -g_j\|^2$. Then for any $\delta>0$, with probability at least $1-\delta$ we have:
\begin{align*}
    \left\| \hat G - G\right\|&\le \sqrt{\frac{8V\log(4d/\delta)}{n}}+\frac{7\log(4d/\delta)\sqrt{2d}}{3(n-1)}
\end{align*}
\end{Theorem}
\begin{proof}
Fix a basis $e_1,\dots,e_d$. For $k=1,\dots,d$, let $\hat G_k=\langle \hat G_k, e_k\rangle$ and $G_k = \langle G_k, e_k\rangle$. Fix some index $k$, and define $x_i = \langle g_i, e_k\rangle$. Then we have $\frac{1}{n}\sum_{i=1}^n x_i = \hat G_k$ and $\frac{1}{n}\sum_{i=1}^n \E[x_i] = G_k$. Define $V_k = \frac{1}{2n(n-1)}\sum_{1\le i<j\le n} (x_i - x_j)^2$. Then by the empirical Bernstein bound, with probability at least $1-\delta/d$ we have:
\begin{align*}
    \left| \hat G_k-G_k\right|\le \sqrt{\frac{4V_k\log(4d/\delta)}{n}}+\frac{7\log(4d/\delta)}{3(n-1)}
\end{align*}
Squaring both sides and using $(a+b)^2\le 2a^2 + 2b^2$, we have:
\begin{align*}
    \left(\hat G_k-G_k\right)^2\le \frac{8V_k\log(4d/\delta)}{n}+\frac{98\log^2(4d/\delta)}{9(n-1)^2}
\end{align*}
Now observe that $V=\sum_{k=1}^d V_k$ and sum the above expression over $k$.
\begin{align*}
    \left|\hat G-G\right|^2\le \frac{8V\log(4d/\delta)}{n}+\frac{98d\log^2(4d/\delta)}{9(n-1)^2}
\end{align*}
Now take square roots and observe that $\sqrt{a+b}\le \sqrt{a}+\sqrt{b}$:
\begin{align*}
    \left|\hat G-G\right|\le \sqrt{\frac{8V\log(4d/\delta)}{n}}+\frac{7\log(4d/\delta)\sqrt{2d}}{3(n-1)}
\end{align*}
\end{proof}


The dimension factor in the above Theorem \ref{thm:dimvariance} is a bit bad. The only reference and proof I know for a similar bound without the dimension is \cite{cutkosky2019combining}, and concentration-via-optimization is probably not the ``right'' way to prove this. Probably there is a better reference out there.
\begin{Theorem}\label{thm:variance}
Suppose $g_1,\dots,g_n$ are i.i.d. samples from a distribution over $d$-dimensional real vectors such that $\|g\|\le 1$ with probability 1. Let $\E[g]=G$, and let $\frac{1}{n}\sum_{i=1}^n g_i = \hat G$. Let $V = \frac{1}{n-1}\sum_{i=1}^n \|g_i-\hat G\|^2=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n} \|g_i -g_j\|^2$. Then for any $\delta>0$, with probability at least $1-\delta$ we have:
\begin{align*}
    \left\| \hat G - G\right\|&\le  O\left(\sqrt{\frac{V\log(n/\delta)}{n}}+\frac{\log(n/\delta)}{n}\right)
\end{align*}
where the big-Oh notation hides absolute constants.
\end{Theorem}


Putting these together, we have the following:
\begin{Theorem}\label{thm:empiricalcovariance}
Suppose $g_1,\dots,g_n$ are i.i.d. samples from a distribution over $d$-dimensional real vectors such that $\|g\|\le 1$ with probability 1. Let $\E[g]=G$, and let $\frac{1}{n}\sum_{i=1}^n g_i = \hat G$. Define the empirical covariance matrix $\hat \Sigma = \frac{1}{n-1}\sum_{i=1}^n (g_i -\hat G)(g_i -\hat G)^\top=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n}(g_i-g_j)(g_i-g_j)^\top$. Let $\sigma^2_1$ be the maximum eigenvalue of $\hat \Sigma$. Let $V = \frac{1}{n-1}\sum_{i=1}^n \|g_i-\hat G\|^2=\frac{1}{2n(n-1)}\sum_{1\le i<j\le n} \|g_i -g_j\|^2$ Then for any $\delta>0$, with probability at least $1-\delta$,
\begin{align*}
    \left| G^\top \hat \Sigma G- \hat G^\top \hat \Sigma \hat G\right| &\le O\left(\frac{\|\hat G\|\sigma^2_1\sqrt{V\log(n/\delta)}}{\sqrt{n}}+\frac{\|\hat G\|\sigma^2_1\log(n/\delta)}{n} +\frac{V\sigma^2_1 \log(n/\delta)}{n} +\frac{\sigma^2_1 \log^2(n/\delta)}{n^2} \right)
\end{align*}
\end{Theorem}
\begin{proof}

Define $\epsilon = G - \hat G$. By Theorem \ref{thm:variance}, we have with probability at least $1-\delta$.
\begin{align*}
\|\epsilon\|&\le O\left(\sqrt{\frac{V\log(n/\delta)}{n}}+\frac{\log(n/\delta)}{n}\right)
\end{align*}
Now we write:
\begin{align*}
    G^\top \hat \Sigma G &= (\hat G + \epsilon)^\top \hat \Sigma(\hat G +\epsilon)\\
    &=\hat G^\top \hat\Sigma \hat G + 2\epsilon^\top \hat \Sigma \hat G + \epsilon^\top \hat \Sigma \epsilon
\end{align*}
We bound the last two terms of the sum individually. First, conditioned on the probability $1-\delta$ event bounding $\epsilon$,
\begin{align*}
    |\epsilon^\top \hat \Sigma \hat G|&\le \sqrt{\epsilon^\top \hat \Sigma \epsilon \hat G^\top \hat \Sigma \hat G}\\
    &\le \|\epsilon\|\sqrt{\sigma^2_1}\sqrt{\hat G^\top \hat\Sigma \hat G}\\
    &\le O\left(\frac{\sqrt{\sigma_ 1V\log(n/\delta)\hat G^\top \hat \Sigma \hat G}}{\sqrt{n}}+\frac{\sqrt{\sigma^2_1 \hat G^\top \hat \Sigma \hat G}\log(n/\delta)}{n}\right)
\end{align*}
and for the second term:
\begin{align*}
    |\epsilon^\top \hat \Sigma \epsilon|&\le \|\epsilon\|^2\sigma^2_1\\
    &\le O\left(\frac{\sigma^2_1 V\log(n/\delta)}{n}+\frac{\sigma^2_1 \log^2(n/\delta)}{n^2}\right)
\end{align*}
where we have used the identity $(a+b)^2\le 2a^2+2b^2$. The full statement now follows by combining these expressions.
\end{proof}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

